SSNet: Saliency Prior and State Space Model-based Network for Salient Object Detection in RGB-D Images

Salient object detection (SOD) in RGB-D images is an essential task in computer vision, enabling applications in scene understanding, robotics, and augmented reality. However, existing methods struggle to capture global dependency across modalities, lack comprehensive saliency priors from both RGB and depth data, and are ineffective in handling low-quality depth maps. To address these challenges, we propose SSNet, a saliency-prior and state space model (SSM)-based network for the RGB-D SOD task. Unlike existing convolution- or transformer-based approaches, SSNet introduces an SSM-based multi-modal multi-scale decoder module to efficiently capture both intra- and inter-modal global dependency with linear complexity. Specifically, we propose a cross-modal selective scan SSM (CM-S6) mechanism, which effectively captures global dependency between different modalities. Furthermore, we introduce a saliency enhancement module (SEM) that integrates three saliency priors with deep features to refine feature representation and improve the localization of salient objects. To further address the issue of low-quality depth maps, we propose an adaptive contrast enhancement technique that dynamically refines depth maps, making them more suitable for the RGB-D SOD task. Extensive quantitative and qualitative experiments on seven benchmark datasets demonstrate that SSNet outperforms state-of-the-art methods.

==> sec/2_lit_review/3_depth.tex <==
\subsection{Uncertain Quality Problems of Depth Maps}
In the RGB-D SOD task, the quality of the depth map plays a crucial role in accurately identifying salient objects. A depth map becomes less effective when the contrast between the salient object and the background is low. However, in real-world scenarios and widely used datasets, depth maps often suffer from quality issues, reducing their reliability. Previous methods have tackled this problem by either discarding low-quality depth maps \cite{impDepth1,impDepth2,dpanet, sip} or estimating depth maps directly from RGB images \cite{cdnet, delving}. Instead of discarding or synthesizing depth information, we propose an adaptive contrast enhancement scheme that refines the original depth map, making it more effective for the RGB-D SOD task.

==> sec/4_results/3_ablation1.tex <==
\subsection{Ablation Study}

The performance of our proposed method depends on the network design of SSNet and the ACE stage. Especially our proposed SSM-based SMDB and CMDB effectively capture the global dependency in intra and inter-modalities. Moreover, the ACE stage enhances the contrast of low-quality depth maps to make them more useful for the SOD task. Additionally, our proposed SEM integrates saliency priors with the deep features from RGB-D images, improving their discriminative capability. In this section, we conduct an ablation study to evaluate the effectiveness of our proposed components. Table \ref{tab:ablation} presents the quantitative results and Figure \ref{fig:ablations_visual} shows the visual comparison of ablation experiments. We first create a baseline model, denoted as "Baseline", by removing ACE, SEM, SMDB, and CMDB from our proposed method. 

\noindent
\textbf{Effectiveness of ACE:} Comparison of results between "Baseline" and "Baseline+ACE" shows that using ACE improves the SOD performance.

\noindent
\textbf{Effectiveness of SEM:} Our novel SEM integrates three saliency priors with the deep features. As evident from the comparison between "Baseline+ACE" and "Baseline+ACE+SEM", the results improve when SEM is used.

\noindent
\textbf{Effectiveness of SMDB:} Our proposed SSM-based SMDB is designed to capture global dependency in self-modality feature maps. Comparison between "Baseline+ACE+SEM" and "Baseline+ACE+SEM+SMDB" shows that the results improve when SMDB is used.

\noindent
\textbf{Effectiveness of CMDB:} Our proposed SSM-based CMDB is designed to capture global dependency between different modality feature maps. Comparison between "Baseline+ACE+SEM+SMDB" and SSNet ("Baseline+ACE+SEM+SMDB+CMDB") shows that the results improve when CMDB is used.

The quantitative and visual comparison results of ablation experiments show that removing any of our proposed components degrades the SOD performance. All these demonstrate the effectiveness of our proposed method.
